Game of Trojans: A Submodular Byzantine Approach

Machine learning models in the wild have been shown to be vulnerable to Trojan attacks during training. Although many detection mechanisms have been proposed, strong adaptive attackers have been shown to be effective against them. In this paper, we aim to answer the questions considering an intelligent and adaptive adversary: (i) What is the minimal amount of instances required to be Trojaned by a strong attacker? and (ii) Is it possible for such an attacker to bypass strong detection mechanisms? We provide an analytical characterization of adversarial capability and strategic interactions between the adversary and detection mechanism that take place in such models. We characterize adversary capability in terms of the fraction of the input dataset that can be embedded with a Trojan trigger. We show that the loss function has a submodular structure, which leads to the design of computationally efficient algorithms to determine this fraction with provable bounds on optimality. We propose a Submodular Trojan algorithm to determine the minimal fraction of samples to inject a Trojan trigger. To evade detection of the Trojaned model, we model strategic interactions between the adversary and Trojan detection mechanism as a two-player game. We show that the adversary wins the game with probability one, thus bypassing detection. We establish this by proving that output probability distributions of a Trojan model and a clean model are identical when following the Min-Max (MM) Trojan algorithm. We perform extensive evaluations of our algorithms on MNIST, CIFAR-10, and EuroSAT datasets. The results show that (i) with Submodular Trojan algorithm, the adversary needs to embed a Trojan trigger into a very small fraction of samples to achieve high accuracy on both Trojan and clean samples, and (ii) the MM Trojan algorithm yields a trained Trojan model that evades detection with probability 1.

==> GameSec2022-references.tex <==


@inproceedings{ji2018transferlearningtrojan,
  title={Model-reuse attacks on deep learning systems},
  author={Ji, Yujie and Zhang, Xinyang and Ji, Shouling and Luo, Xiapu and Wang, Ting},
  booktitle={Proceedings {ACM} {C}onference on {C}omputer and {C}ommunications {S}ecurity},
  pages={349--363},
  year={2018}
}

@inproceedings{goodfellow2015explain,
title	= {Explaining and Harnessing Adversarial Examples},
author	= {Ian Goodfellow and Jonathon Shlens and Christian Szegedy},
year	= {2015},
booktitle	= {International Conference on Learning Representations}
}

@inproceedings{yao2019latent,
  title={Latent backdoor attacks on deep neural networks},
  author={Yao, Yuanshun and Li, Huiying and Zheng, Haitao and Zhao, Ben Y},
  booktitle={ACM SIGSAC Conference on Computer and Communications Security},
  pages={2041--2055},
  year={2019}
}

@article{shafahi2018poison,
  title={Poison frogs! {T}argeted clean-label poisoning attacks on neural networks},
  author={Shafahi, Ali and Huang, W Ronny and Najibi, Mahyar and Suciu, Octavian and Studer, Christoph and Dumitras, Tudor and Goldstein, Tom},
  journal={Advances in {N}eural {I}nformation {P}rocessing {S}ystems},
  volume={31},
  year={2018}
}

@inproceedings{rakin2020tbt,
  title={T{BT}: Targeted neural network attack with bit {T}rojan},
  author={Rakin, Adnan Siraj and He, Zhezhi and Fan, Deliang},
  booktitle={IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={13198--13207},
  year={2020}
}


@article{goodfellow2014generative,
  title={Generative adversarial nets},
  author={Goodfellow, Ian and Pouget-Abadie, Jean and Mirza, Mehdi and Xu, Bing and Warde-Farley, David and Ozair, Sherjil and Courville, Aaron and Bengio, Yoshua},
  journal={Advances in {N}eural {I}nformation {P}rocessing {S}ystems},
  volume={27},
  year={2014}
}

@inproceedings{xu2021detecting,
  title={Detecting {AI} {T}rojans using meta neural analysis},
  author={Xu, Xiaojun and Wang, Qi and Li, Huichen and Borisov, Nikita and Gunter, Carl A and Li, Bo},
  booktitle={IEEE Symposium on Security and Privacy (SP)},
  pages={103--120},
  year={2021},
  organization={}
}

@article{BiaMirBuh-16,
  title={Guaranteed non-convex optimization: Submodular maximization over continuous domains},
  author={Bian, Andrew An and Mirzasoleiman, Baharan and Buhmann, Joachim M and Krause, Andreas},
  journal={International Conference on Artificial Intelligence and Statistics},
  pages={111--120},
  year={2017}
}

@article{bach2016submodular,
  title={Submodular functions: {F}rom discrete to continuous domains},
  author={Bach, Francis},
  journal={Mathematical Programming},
  pages={1--41},
  year={2016},
  publisher={Springer}
}



@inproceedings{dumford2020backdooring,
  title={Backdooring convolutional neural networks via targeted weight perturbations},
  author={Dumford, Jacob and Scheirer, Walter},
  booktitle={International Joint Conference on Biometrics},
  pages={1--9},
  year={2020},
  organization={IEEE}
}

@article{tran2018spectral,
  title={Spectral signatures in backdoor attacks},
  author={Tran, Brandon and Li, Jerry and Madry, Aleksander},
  journal={Advances in {N}eural {I}nformation {P}rocessing {S}ystems},
  volume={31},
  year={2018}
}

@article{chan2019poison,
  title={Poison as a cure: Detecting \& neutralizing variable-sized backdoor attacks in deep neural networks},
  author={Chan, Alvin and Ong, Yew-Soon},
  journal={arXiv preprint arXiv:1911.08040},
  year={2019}
}

@InProceedings{hayase2021spectre,
  title = 	 {{SPECTRE}: defending against backdoor attacks using robust statistics},
  author =       {Hayase, Jonathan and Kong, Weihao and Somani, Raghav and Oh, Sewoong},
  booktitle = 	 {38th International Conference on Machine Learning},
  pages = 	 {4129--4139},
  year = 	 {2021},
  volume = 	 {139},
  series = 	 {Proceedings of Machine Learning Research},
  month = 	 {18--24 Jul},
  publisher =    {PMLR},
}


@inproceedings{wang2019neural,
  title={Neural cleanse: {I}dentifying and mitigating backdoor attacks in neural networks},
  author={Wang, Bolun and Yao, Yuanshun and Shan, Shawn and Li, Huiying and Viswanath, Bimal and Zheng, Haitao and Zhao, Ben Y},
  booktitle={IEEE Symposium on Security and Privacy (SP)},
  pages={707--723},
  year={2019},
  organization={}
}

@article{guo2019tabor,
  title={T{ABOR}: {A} highly accurate approach to inspecting and restoring {T}rojan backdoors in {AI} systems},
  author={Guo, Wenbo and Wang, Lun and Xing, Xinyu and Du, Min and Song, Dawn},
  journal={arXiv preprint arXiv:1908.01763},
  year={2019}
}

@article{huang2019neuroninspect,
  title={Neuron{I}nspect: {D}etecting backdoors in neural networks via output explanations},
  author={Huang, Xijie and Alzantot, Moustafa and Srivastava, Mani},
  journal={arXiv preprint arXiv:1911.07399},
  year={2019}
}
@inproceedings{chen2019deepinspect,
  title={DeepInspect: A Black-box {T}rojan Detection and Mitigation Framework for Deep Neural Networks.},
  author={Chen, Huili and Fu, Cheng and Zhao, Jishen and Koushanfar, Farinaz},
  booktitle={IJCAI},
  volume={2},
  pages={8},
  year={2019}
}

@inproceedings{kolouri2020universal,
  title={Universal litmus patterns: Revealing backdoor attacks in {CNN}s},
  author={Kolouri, Soheil and Saha, Aniruddha and Pirsiavash, Hamed and Hoffmann, Heiko},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={301--310},
  year={2020}
}

@inproceedings{krizhevsky2012imagenet,
  title={Imagenet classification with deep convolutional neural networks},
  author={Krizhevsky, Alex and Sutskever, Ilya and Hinton, Geoffrey E},
  booktitle={Advances in {N}eural {I}nformation {P}rocessing {S}ystems},
  volume={25},
  year={2012}
}

@article{stallkamp2012man,
  title={Man vs. computer: Benchmarking machine learning algorithms for traffic sign recognition},
  author={Stallkamp, Johannes and Schlipsing, Marc and Salmen, Jan and Igel, Christian},
  journal={Neural networks},
  volume={32},
  pages={323--332},
  year={2012},
  publisher={Elsevier}
}

@article{bian2017continuous,
  title={Continuous {DR}-submodular maximization: Structure and algorithms},
  author={Bian, An and Levy, Kfir and Krause, Andreas and Buhmann, Joachim M},
  journal={Advances in {N}eural {I}nformation {P}rocessing {S}ystems},
  volume={30},
  year={2017}
}

@inproceedings{liu2017neural,
  title={Neural {T}rojans},
  author={Liu, Yuntao and Xie, Yang and Srivastava, Ankur},
  booktitle={International Conference on Computer Design},
  pages={45--48},
  year={2017},
  organization={IEEE}
}

@inproceedings{liu2018fine,
  title={Fine-pruning: {D}efending against backdooring attacks on deep neural networks},
  author={Liu, Kang and Dolan-Gavitt, Brendan and Garg, Siddharth},
  booktitle={International Symposium on Research in Attacks, Intrusions, and Defenses},
  pages={273--294},
  year={2018},
  organization={Springer}
}

@article{rajabi2022trojan,
  title={Trojan Horse Training for Breaking Defenses against Backdoor Attacks in Deep Learning},
  author={Rajabi, Arezoo and Ramasubramanian, Bhaskar and Poovendran, Radha},
  journal={arXiv preprint arXiv:2203.15506},
  year={2022}
}

@article{rajabi2022ByzGame,
  title={Byzantine Game of Trojans},
  author={Rajabi, Arezoo and others},
  journal={arXiv preprint XYZ},
  year={2022}
}

@inproceedings{koh2017understanding,
  title={Understanding black-box predictions via influence functions},
  author={Koh, Pang Wei and Liang, Percy},
  booktitle={International conference on machine learning},
  pages={1885--1894},
  year={2017},
  organization={PMLR}
}


@INPROCEEDINGS{helber2019eurosat,
  author={Helber, Patrick and Bischke, Benjamin and Dengel, Andreas and Borth, Damian},
  booktitle={IEEE International Geoscience and Remote Sensing Symposium}, 
  title={Introducing {E}uro{SAT}: A Novel Dataset and Deep Learning Benchmark for Land Use and Land Cover Classification}, 
  year={2018},
  volume={},
  number={},
  pages={204-207},
}


@inproceedings{yoshida2020disabling,
  title={Disabling backdoor and identifying poison data by using knowledge distillation in backdoor attacks on deep neural networks},
  author={Yoshida, Kota and Fujino, Takeshi},
  booktitle={ACM Workshop on Artificial Intelligence and Security},
  pages={117--127},
  year={2020}
}

@TECHREPORT{krizhevsky2009CIFARs,
    author = {Alex Krizhevsky},
    title = {Learning multiple layers of features from tiny images},
    institution = {University of Toronto},
    year = {2009}
}

@inproceedings{guo2022aeva,
  title={A{EVA: B}lack-box Backdoor Detection Using Adversarial Extreme Value Analysis},
  author={Guo, Junfeng and Li, Ang and Liu, Cong},
  booktitle={International Conference on Learning Representations},
  year={2022}
}

@article{li2021neural,
  title={Neural attention distillation: Erasing backdoor triggers from deep neural networks},
  author={Li, Yige and Lyu, Xixiang and Koren, Nodens and Lyu, Lingjuan and Li, Bo and Ma, Xingjun},
  journal={International Conference on Learning Representations},
  year={2021}
}

@article{ullah2019cyber,
  title={Cyber security threats detection in {IoT} using deep learning approach},
  author={Ullah, Farhan and Naeem, Hamad and Jabbar, Sohail and Khalid, Shehzad and Latif, Muhammad Ahsan and Al-Turjman, Fadi and Mostarda, Leonardo},
  journal={IEEE Access},
  volume={7},
  pages={},
  year={2019},
  publisher={IEEE}
}

@article{gu2019badnets,
  title={Bad{N}ets: {E}valuating backdooring attacks on deep neural networks},
  author={Gu, Tianyu and Liu, Kang and Dolan-Gavitt, Brendan and Garg, Siddharth},
  journal={IEEE Access},
  volume={7},
  pages={47230--47244},
  year={2019},
  publisher={IEEE}
}

@misc{AWS,
  title = {Amazon, {M}achine learning at {AWS}, 2018.}
}

@misc{Caffe,
  title = {Caffe, {C}affe {M}odel {Z}oo, 2018.}
}

@misc{BigML,
  title = {Big{ML} {I}nc. {Big}{ML}, 2018}
}

@article{bojarski2016end,
  title={End to end learning for self-driving cars},
  author={Bojarski, Mariusz and Del Testa, Davide and Dworakowski, Daniel and Firner, Bernhard and Flepp, Beat and Goyal, Prasoon and Jackel, Lawrence D and Monfort, Mathew and Muller, Urs and Zhang, Jiakai and Zhang, Xin and Zhao, Jake and Zieba, Karol},
  journal={arXiv preprint arXiv:1604.07316},
  year={2016}
}

@article{silver2016mastering,
  title={Mastering the game of {G}o with deep neural networks and tree search},
  author={Silver, David and Huang, Aja and Maddison, Chris J. and Guez, Arthur and Sifre, Laurent and van den Driessche, George and Schrittwieser, Julian and Antonoglou, Ioannis and Panneershelvam, Veda and Lanctot, Marc and Dieleman, Sander and Grewe, Dominik and Nham, John and Kalchbrenner, Nal and Sutskever, Ilya and Lillicrap, Timothy and Leach, Madeleine and Kavukcuoglu, Koray and Graepel, Thore and Hassabis, Demis},
  journal={Nature},
  volume={529},
  number={7587},
  pages={484--489},
  year={2016},
  publisher={Nature Publishing Group}
}

@article{esteva2019guide,
  title={A guide to deep learning in healthcare},
  author={Esteva, Andre and Robicquet, Alexandre and Ramsundar, Bharath and Kuleshov, Volodymyr and DePristo, Mark and Chou, Katherine and Cui, Claire and Corrado, Greg and Thrun, Sebastian and Dean, Jeff},
  journal={Nature Medicine},
  volume={25},
  number={1},
  pages={24--29},
  year={2019},
  publisher={Nature Publishing Group}
}

@article{sarkar2020backdoor,
  title={Backdoor suppression in neural networks using input fuzzing and majority voting},
  author={Sarkar, Esha and Alkindi, Yousif and Maniatakos, Michail},
  journal={IEEE Design \& Test},
  volume={37},
  number={2},
  pages={103--110},
  year={2020},
  publisher={IEEE}
}

@inproceedings{gao2019strip,
  title={Strip: A defence against trojan attacks on deep neural networks},
  author={Gao, Yansong and Xu, Change and Wang, Derui and Chen, Shiping and Ranasinghe, Damith C and Nepal, Surya},
  booktitle={Proceedings of the 35th Annual Computer Security Applications Conference},
  pages={113--125},
  year={2019}
}


@article{gao2020backdoor,
  title={Backdoor attacks and countermeasures on deep learning: A comprehensive review},
  author={Gao, Yansong and Doan, Bao Gia and Zhang, Zhi and Ma, Siqi and Zhang, Jiliang and Fu, Anmin and Nepal, Surya and Kim, Hyoungshick},
  journal={arXiv preprint arXiv:2007.10760},
  year={2020}
}

@article{lecun1998mnist,
  title={The {MNIST} database of handwritten digits},
  author={LeCun, Yann},
  journal={http://yann. lecun. com/exdb/mnist/},
  year={1998}
}

@inproceedings{GTSRB013,
   author = {Sebastian Houben and Johannes Stallkamp and Jan Salmen and Marc Schlipsing and Christian Igel},
   booktitle = {International Joint Conference on Neural Networks},
   title = {Detection of Traffic Signs in Real-World Images: The {G}erman {T}raffic {S}ign {D}etection {B}enchmark},
   number = {1288},
   year = {2013},
}

@inproceedings{he2016resnet,
  title={Deep residual learning for image recognition},
  author={He, Kaiming and Zhang, Xiangyu and Ren, Shaoqing and Sun, Jian},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={770--778},
  year={2016}
}

@article{hinton2015distilling,
  title={Distilling the knowledge in a neural network},
  author={Hinton, Geoffrey and Vinyals, Oriol and Dean, Jeff and others},
  journal={arXiv preprint arXiv:1503.02531},
  volume={2},
  number={7},
  year={2015}
}

@inproceedings{shen2021backdoor,
  title={Backdoor scanning for deep neural networks through k-arm optimization},
  author={Shen, Guangyu and Liu, Yingqi and Tao, Guanhong and An, Shengwei and Xu, Qiuling and Cheng, Siyuan and Ma, Shiqing and Zhang, Xiangyu},
  booktitle={International Conference on Machine Learning},
  pages={9525--9536},
  year={2021},
  organization={PMLR}
}

@inproceedings{panagiota2020trojdrl,
  title={Troj{DRL}: {T}rojan Attacks on Deep Reinforcement Learning Agents},
  author={Panagiota, Kiourti and Kacper, Wardega and Jha, Susmit and Wenchao, Li},
  booktitle={ACM/IEEE Design Automation Conference},
  year={2020}
}

@article{mnih2015DQN,
  title={Human-level control through deep reinforcement learning},
  author={Mnih, Volodymyr and Kavukcuoglu, Koray and Silver, David and Rusu, Andrei A and Veness, Joel and Bellemare, Marc G and Graves, Alex and Riedmiller, Martin and Fidjeland, Andreas K and Ostrovski, Georg and others},
  journal={nature},
  volume={518},
  number={7540},
  pages={529--533},
  year={2015},
  publisher={Nature Publishing Group}
}
